A Study of Library Migration in Java Software

Software intensively depends on external libraries whose relevance may change during its life cycle. As a consequence, software developers must periodically reconsider the libraries they depend on, and must think about \textit{library migration}. To our knowledge, no existing study has been done to understand library migration although it is known to be an expensive maintenance task. Are library migrations frequent? For which software are they performed and when? For which libraries? For what reasons? The purpose of this paper is to answer these questions with the intent to help software developers that have to replace their libraries. To that extent, we have performed a statistical analysis of a large set of open source software to mine their library migration. To perform this analysis we have defined an approach that identifies library migrations in a pseudo-automatic fashion by analyzing the source code of the software. We have implemented this approach for the Java programming language and applied it on Java Open Source Software stored in large hosting services. The main result of our study is that library migration is not a frequent practice but depends a lot on the nature of the software as well as the nature of the libraries.

==> algorithm.tex <==
\section{Approach}
\label{sec:approach}

\newtheorem{thm}{Theorem}
\newtheorem{definition}{Definition}

In this section, we first present the abstract model we define to represent software and library migrations. Based on this model, we present the approach we propose to identify library migrations. 

\subsection{Dependency Model}

We abstract the data needed to perform our analysis in a dependency model. This model is very simple as it only contains the set of analysed software, their list of versions and, for each version the associated set of library dependencies. 

\begin{definition}[Software and Libraries]
Let $S$ be the set of software and $L$ be the set of libraries. 
For the sake of simplicity, we consider that each software $s \in S$ has an associated totally ordered set $V_s \subset \mathds{N}$ of versions. Versions are sorted chronologically according to their date. 
For a software $s \in S$ at version $i \in V_s$, we define $dep_s(i) : V_s \rightarrow {\cal S}(L)$ the set of its library dependencies.
\label{def:projects-libraries}
\end{definition}

Let us illustrate our model with an example. We assume two software ($\mathtt{S_A}$ and $\mathtt{S_B}$) and four libraries (\lib{JUnit}, \lib{TestNG}, \lib{Log4J} and \lib{SLF4J}). Table \ref{tab:dependency-model} presents this dependency model with version of $\mathtt{S_A} : (1, 2, 3))$ and of $\mathtt{S_B} : (1, 2)$, associated with their corresponding dependencies. Note that versions $1$ of $\mathtt{P_A}$ and version $1$ of $\mathtt{P_B}$ are different and occur at two different dates. 

\begin{table}
\centering
\scriptsize
\begin{tabular}{cccc}
\toprule
Software & \multicolumn{3}{c}{Versions / Dependencies}\\
\midrule
$\mathtt{S_A}$ & $1$ & $2$ & $3$\\
& $\{$\texttt{JUnit}$\}$ & $\{$\texttt{JUnit},\texttt{TestNG},\texttt{Log4J}$\}$& $\{$\texttt{TestNG},\texttt{SLF4J}$\}$\\
\midrule
$\mathtt{S_B}$ & $1$ & $2$ & \\
& $\{$\texttt{TestNG}$\}$ & $\{$\texttt{JUnit}$\}$&\\
\bottomrule
\end{tabular}
\caption{Example of 2 software with their versions and their dependencies}
\label{tab:dependency-model}
\end{table}

\begin{definition}[Library migration]
We state that a software $s \in S$ migrates from an old library $o \in L$ to new one $n \in L$ if it depends on $o$ at version $i \in V_s$ (i.e. $o \in dep_s(i)$) and if it replaces this dependency by $n \in L$ in version $j \in V_s$ with $i < j$ (i.e. $n \in dep_s(j)$). A migration is therefore a tuple $(s,i,j,o,n) \in S \times \mathds{N} \times \mathds{N} \times L \times L$. Finally, given a set of software $S$ and a set of libraries $L$, we note $M$ all the migrations that occur for all software in $S$.
\label{def:library-migration}
\end{definition}


Regarding our sample presented in Table \ref{tab:dependency-model}, the following migrations have been performed in software $S_A$ and $S_B$: $(S_A,1,3,junit,testng)$, $(S_A,2,3,log4j,slf4j)$ and $(S_B,1,2,testng,junit)$. 

\begin{definition}[Library migration rule]
We also call a migration rule a couple $(o,n) \in L^2$ such that there exists at least one software $s \in P$ that migrates from $o$ to $n$ during its life-cycle. We note $R$ the set of all library migration rules.
\label{def:library-migration-rule}
\end{definition}


Regarding our example $R=\{(junit,testng), (log4j , slf4j), (testng , junit)\}$.


\subsection{Mining library migrations}

To answer our research questions, we have to identify migrations $M$ that occur in a set of software $S$ for a set of libraries $L$. Such an identification obviously first requires to define $S$ but also $L$. While defining $S$ is trivial, defining $L$ is not so obvious and mainly depends on the programming language. \secref{study} presents how we manage to identify $S$ and $L$ for Java Open Source software.

Once $S$ and $L$ have been defined, our approach has to define how library dependencies can be automatically computed (the $dep_s(i)$ function has to be defined). To that extent, several techniques can be used such as the ones that are based on tools that manage library dependencies like Maven for instance~\cite{teyton_mining_2012}. In this paper, we choose not to depend on a specific tool but rather to use source code static analysis for computing automatically dependencies between a software and a set of libraries. \secref{study} presents such a simple static analysis for Java software and Java libraries.

Further, to compute $M$, we propose an algorithm that iterates on several versions of each software to identify migrations that have been performed. In detail, our algorithm looks at couples of versions $(i,j)$ in a software $s$ and checks which library dependencies existed at version $i$ but were replaced at version $j$. Our algorithm proposes a candidate migration for each element of the Cartesian product between the dependencies that existed at $i$ but were removed at $j$ and the ones that did not exist at $i$ but were added at $j$. 

With our example, considering the software $S_A$ and the couple of versions $(1,3)$, our algorithm proposes the candidates $(S_A,1,3,junit,testng)$ and $(S_A,1,3,junit,slf4j)$. Considering the same software but the couple of version $(1,3)$, our algorithm proposes the candidates $(S_A,1,3,junit,testng)$ and $(S_A,1,3,junit,slf4j)$.

The choice of couples $(i,j)$ to observe has a major impact on the quantity of the candidate migrations returned by our algorithm. Ideally all couples should be observed to get all possible candidates but this takes too much time and is certainly not useful as many couples return the same migrations. Further, the choice of the distance between the two versions of the couple ($j-i$) has also an impact on the returned candidates. The following two cases should be considered: 
	\begin{itemize}
		\item \textit{Large} distance couples ($(j-i)$ approaches to $\infty$). If the distance between the couple is too large, several migrations that occur between $i$ and $j$ will not be considered to be candidate. The \figref{largeDistanceCouple} presents four situations in which such a case may occur. In this figure, an horizontal axis represents a dependency toward a certain kind of library for a given software (for instance a dependency toward a testing library). Each coloured segment displays which library has been used as a dependency (e.g. $junit$ then $testng$) and thus also displays when migrations occurred (\textcircled{m}). Each of the four cases represents completely different situations which are:  %if the migrated library is added after $i$ or if there is an inverse migration that occurs before $j$.
			\begin{enumerate}
				\item The introduction of $junit$ was done after $i$, hence by observing the couple $(i,j)$ our algorithm does not know that $junit$ was used before $testng$ and therefore won't return any candidate.
				\item The software stopped to use $testng$  before $j$, thus by observing the couple $(i,j)$ our algorithm does not know $testng$ and therefore won't return any candidate. 
				\item Two migrations happened between $i$ and $j$. $junit$ was replaced by $TestNG$ that was then by $jetty-test$. Here, by observing the couple $(i,j)$ our algorithm will consider only the candidate $(i,j,junit,jetty-test)$, which never occurs.
				\item The software migrated from $junit$ to $testng$ between $i$ and $j$, but then moved back to $junit$ before the version $j$. By observing the couple $(i,j)$ our algorithm won't return any candidate.
			\end{enumerate}	 
		\item \textit{Small} distance couples ($(j-i)$ approaches to $1$). If the distance between the couple is too small, migrations that are performed during several versions won't be detected. As a matter of fact a migration might not always be performed during only one version. The new dependency might be added at version $j$ but the old one might be kept at version $j$ and be removed lately at $j+k$. Our example highlights such a situation with the project $S_A$. In particular, if our algorithm observes the couple of versions $(1,2)$ and $(2,3)$, the candidate $(S_A,1,3,junit,testng)$ won't be returned.
	\end{itemize}
	
	\begin{figure}[h]
		\centering
        \includegraphics[width=0.9\linewidth]{pics/jsep/largeDistanceCouple.pdf}
        \caption{Cases of migrations missed if the distance between the versions couple is too large}
		\label{fig:largeDistanceCouple}
	\end{figure}



The choice of the couples to observe and their distance therefore requires to reach a trade-off between the quantity of returned migrations and time efficiency. \secref{study} presents a discussion about this trade-off for Open Source Java projects.


Whatever the number of observed couples of versions and whatever their distance, once candidate migrations have been identified, they have to be validated either automatically or manually before to be truly included in $M$, the set of migrations. Regarding our example, the candidate $(S_A,1,3,junit,slf4j)$ should be filtered out while $(S_A,1,3,junit,testng)$ should be filtered in. \secref{study} explains that, although an automatic validation provided good results in our previous study, it has a very bad recall for our currently study and this is why we therefore have realized a manual validation. 


\subsection{Methodology to answer the research questions}
\paragraph{In which projects migrations are performed?}

To identify if some kinds of projects are prone to migration, we choose to use metrics to statistically measure the size of projects and to compare it with the number of performed migrations.

We arbitrary choose three metrics that are classically used to measure the size of a project: KLOC, Commit and Duration. In our study, the KLOC metric computes the number of lines of Java code. The Commit metric measures the number of commits that were performed during the life of the project. The Duration metric measures the life time of the project in months. 

Once we have measured these three metrics for all the projects we decided to remove: all projects that have less than 100 KLOC, the ones that have less than 10 commits and the ones that are younger than one month. Our intent was to remove all toy projects that are not significant regarding library migrations.

Finally, we decided to compute deciles for each metric in order to define groups of projects with similar size. Then we have measured the number of migrations for each group and we have performed a chi-squared test to check if the distribution of migrations is the same for all groups for each metric.

If the distribution is not the same, we plot the distributions of the groups for each metric to observe how the number of migrations varies depending on the metric.



\paragraph{Which library are prone to migration?}

%After having identified migration rules and self loops,  

To identify if there are libraries that are prone to migration, we choose to group libraries that are connected by migration rules. To that extent we compute what we call a migration graph. The nodes of this graph are libraries that have been either source or target of at least one migration. A directed arc exists between two nodes if there is at least a migration between the two nodes. To indicate the flow of migration between the different libraries, the arcs are  by the number of migrations that have been observed for the libraries source and target of the arcs. We then compute the connected components on the migration graph. Each connected component is a category, whose libraries of the category are the union of the libraries contained in the connected component. 

An example of category is shown in~\figref{migrationgraph}. This category shows that \lib{JUnit} and \lib{TestNG} are similar and that projects have performed migration in the both sides. Note that such migration graph does not mention if the same project made the two migrations or if it is two distinct projects. 

\begin{figure}[h]
\centering
\includegraphics[width=0.45\linewidth]{pics/sample_migration_graph.pdf}
\caption{A category formed in our example}
\label{fig:migrationgraph}
\end{figure}

A category exhibits a set of similar libraries but also the number of migrations that have been performed between them. 

We define for a library $l$ the \textit{introductions} value as the number of times any project $p \in P$ started to use $l$. This is a more representative view of the actual usage of $l$ through several years and allows to measure more precisely the proportion of library usage that led to a migration. Given a category, the \textit{introductions} value corresponds to the sum of the \textit{introductions} of each of its libraries.

We can then compare the number of migrations of a category with the number of library \textit{introductions} of the category. Such a ratio indicates if the category is prone to migration. 

As a complement, we introduce the popularity-evolution diagram. For a given category, it displays the evolution of the number of client projects of each library in the category. This number is computed every 2 weeks on a defined period of time. An example of such diagram is exposed in \figref{usage-diagram}. A migration is characterized in this context by a loss of client for the source library and a client gain for the target library. Note that the number of \textit{introductions} in \figref{usage-diagram} is 5 for \lib{JUnit} and 3 for \lib{TestNG}, and thus 8 for the category.

\begin{figure}[h]
\centering
\includegraphics[width=0.55\linewidth]{pics/jsep/popularity_sample.pdf}
\caption{An example of popularity-evolution diagram}
\label{fig:usage-diagram}
\end{figure}


\paragraph{When migration are performed?}

To check if the date has any influence on migrations, we compute what we call a migration-time diagram. A migration-time diagram targets one given category of library and presents the dates of all the migrations that happened in this category. The x-axis of the diagram presents the chronological time. The y-axis is decomposed of as much as existing migration rules in the category. A point in a diagram represents a migration. This diagram allows to visualize and detect if a migration is associated to a time period, and the respective trends for the source and the target as well.
%Note that the position in time for a migration $(p,i,j,s,t)$ is the middle position between the dates of resp. $i$ and $j$ for the project $p$. Thus, dates are approximations only.

Figure \ref{fig:migration-time-diagram} presents a sample migration-time diagram for the category formed in our example. This diagram is just a toy diagram that highlights the two migrations.

\begin{figure}[h]
\centering
\includegraphics[width=0.55\linewidth]{pics/jsep/testing_sample.pdf}
\caption{An example of migration-time diagram for the \textit{JUnit} $\rightarrow$ \textit{TestNG} migration}
\label{fig:migration-time-diagram}
\end{figure}


\paragraph{Why migration are performed?}

To identify why developers perform migrations, we decided to manually review commits logs recorded between each couple of project versions \textit{(i,j)} that contain a migration $(p,i,j,s,t)$. If a justification is provided in the message, we picked up the log and we tried to label it with an arbitrary category of motivation. The goal is to propose a taxonomy of the motivations found.

An example of commit log of interest found on the Web is \textsl{"port logging to Slf4J (Commons-logging has classloader issues)}''\footnote{http://code.google.com/p/dyuproject/source/detail?r=668} and designates a migration that dropped a library due to a running issue. This technique is however dependent on the quality of commit messages written by developers. 


\paragraph{How migrations are performed?}

To measure the time needed to perform a migration $(p,i,j,s,t)$, we compute the time when $s$ has been removed ($t_{rem}$) and the time when $t$ has been introduced ($t_{add}$). We then measure how many commits were needed between $t_{rem}$ and $t_{add}$, how many developers were involved, and how many \textit{commits} days were counted. A \textit{commit} day is simply a calendar day where a commit has been registered. 

The goal of this analysis is to measure the developers efforts and common habits during a migration. The results will quantify the number of migrations achieved between two commits, i.e. the shortest interval of time, and those accomplished through at least two commits. This situation reveals period of coexistence of the source and target libraries. 

If more that one version is needed, it may be due to painful efforts and particular adaptations made to the source code. We will try to extract this information through commit logs, projects issue trackers or mailing lists.


==> maven.tex <==
\section{Backgrounds}\label{sec:maven}

This section introduces the reader to Maven and the reasons why we choose this a study case.

\subsection{Apache Maven}

Apache Maven\footnote{http://maven.apache.org/} is a build automation tool that uses a POM (Project Object Model) mandatory XML file where the software project is described. This file lists the plug-ins and dependencies used and specifies how the project must be compiled and built. It has the particularity to dynamically downloads dependencies, which are stored on a central repository. Thus, each dependency must be carefully identified and its version number as well. Each Maven element is named as an artifact. An artifact is described by three elements : a \emph{groupId} (e.g. organization name, company name), an \emph{artefactId} (the unique name of the library under the \emph{groupId}), and the specific release chosen, the \emph{version}. This triplet represents a consistent information that uniquely identify an artifact. This is the reason why we avoid projects where libraries are stored on the repository and do not necessary provide data on their version release. For example, a file "junit.jar" lacks information. 
An example of dependency specification with Maven is shown in Figure \ref{fig:mvnDep}. The \emph{version} element is not mandatory in this step. Indeed, Maven will consider the most recent version of the artifact.

\begin{figure}
\centering
\includegraphics[width=0.65\linewidth]{pics/dep_specif.pdf}
\caption{A sample of dependency specification in POM.xml file}
\label{fig:mvnDep}
\end{figure}

\subsection{Maven Central Repository}

When Maven compiles a project, it needs to retrieve each dependency from a Maven repository.  These dependencies are actually Maven projects that are packaged and stored on such repositories. They become therefore available for usage, as only their identity have to be specified in POM files. Moreover, each POM file contains the URL address of the repository where the required artifacts can be found. Usually, those artefacts are deposited with both source and binary files,  and their POM file is included as well. The architecture of Maven repositories allows to classify artifacts by their respective \emph{groupId}, \emph{artifactId} and \emph{version}. Thus, it becomes possible to identify the list of versions of a given artifact by the combination of both its \emph{groupId} and \emph{artifactId}. We can then perform a comparison of the successive versions of the POM files. Maven Central Repository references currently about 310 000 unique artifacts and is the most popular repository. It serves over 70 millions downloads every week\footnote{http://www.sonatype.com/people/2010/12/now-available-central-download-statistics-for-oss-projects/}.

\subsection{Lacks for recommendation}

The Repository proposes a search engine based on textual inputs. In this way, any developer can look up for a dependency based on the \emph{groupId} and/or \emph{artifactId}. As mentioned in Section \ref{sec:intro}, it happens that artifact become henceforth maintained under a new \emph{groupId}. We do not consider this situation as a \emph{migration}, since the object is the same but owns a new identity. Also, any developer can use the search engine to find a specific \emph{artifactId} and check which is the most recent released, and hence the correlated \emph{groupId}. We discard this case as it does not enhance any problem. 

We stipulate a lack exists currently when a developer looks for a replacement library. Indeed, as similar APIs are not established, it is tricky to find an API based on keywords only. The features or the category of an API is not necessary represented in its name. Moreover, even a developer finds results, nothing indicates how much popular and relevant is each candidate found. For example, if an API name contains "SQL", no one can claim this is a database system or a query utils tool for instance. On the contrary, a developer using an the library \emph{MySQL} is ensured that a significant migration rate between \emph{MySQL} and \emph{HSQLDB} indicates that the two libraries can be used for the same purpose. 
  
We laid down the backgrounds about \textsc{Maven} and we need now a process to study the artifact evolutions. 

==> rules.tex <==
\section{Mining Migration Rules}\label{sec:rules}

In this section we expose the process following the data set generation from Maven Central Repository mining. We detail how the histories are analyzed to produce the data structure that contain the \emph{migration} rules. 

\subsection{Rule generation algorithm}\label{sec:rules_gen}

For each Maven artifact, we explained how to compute the history of its dependencies specified in the POM file. An history is a set of operations that represent dependencies additions and removals so that switching can be detected. The purpose is henceforth to compute each of these histories independently and to output a list of \emph{migration} rules. A \emph{migration} rule $(s,t)$ is created when a deletion of an artifact $s$ and addition of an artifact $t$ is observed for the first time. This obviously does not necessarily mean that such fact corresponds to a change of API of same purposes. This is why we count the number of times a rule $(s,t)$ is generated. A data structure \textsc{score} stores and counts the number of occurrence of each of the rule. 

We argue that a \emph{migration} rule makes sense if observed within more than one organization, that is more than one distinct \emph{groupId}. Indeed, under a unique \emph{groupId}, several artifacts may undergo an identical API change. This is generally a move decided by the same group of persons that apply a common policy. A second data structure \textsc{groups} maintains for each rule the distincts \emph{groupId} of artifacts under which a \emph{migration} rule was observed.

For each artifact $a \epsilon A$, once the history is built, queries are performed to extract a list of \emph{migration} rule. A query is executed for every $D_a^v$ found in the history of \emph{a}. This seeks for both removed and added dependencies during this \emph{diff}. Migration rules are built by proceeding to a cartesian product of the two retrieved sets. For each rule found, the structures \textsc{SCORE} and \textsc{GROUPS} are maintained . 

These queries are written in Prolog using the engine SWI-Prolog\footnote{www.swi-prolog.org/} engine.

 Finally, a score is obtained for the \emph{migration} rules. We can thus obtain a list of rules sorted on the score in order to highlight the most relevant data. To that purpose, we need some filtering rules to discard false positives. 

\subsection{Rule filtering}

\subsubsection{During the computation}

The first filter is applied during the cartesian product between the removed and added dependencies. Indeed, we need to discard artefacts involved in any couple (\emph{s,t}) of artifacts when $s$ and $t$ are judged equivalent. This betides in two cases :
\begin{itemize}
\item The \emph{groupId} of $s$ and $t$ are equivalent. 
\item Consider ${aid}_s$ and ${aid}_t$ the lexical tokens of the \emph{artifactId} of $s$ (resp. $t$), dissociated by any punctuation. If ${aid}_s \cap {aid}_t \neq \emptyset$, they is a similarity.
\end{itemize}

To make it clear, consider the following example. A couple \texttt{(org.junit.junit,junit.junit-dep)} is detected during a \emph{diff} analysis. The \emph{groupId} \texttt{org.junit} and \texttt{junit} are not similar. However, the tokens through the \emph{artifactId} are respectively \texttt{\{"junit"\}} and \texttt{\{"junit","dep"\}}. As the intersection is not empty

\begin{figure}
\scriptsize
\begin{algorithmic}[1] 
\STATE $\textsc{score} \gets \emptyset$ \COMMENT{\textit{Map of rules with score associated}}
\STATE $\textsc{groups} \gets \emptyset$ \COMMENT{\textit{Map of rules with groupIds associated}}
\FORALL {$artf \in A$}
		\FORALL {$D_{artf}^{v} \in History_{artf}$}
		\STATE $a_{rem} \gets D_{artf}^{v}.getRemovedDep()$
		\STATE $a_{add} \gets D_{artf}^{v}.getAddedDep()$
		\STATE $related \gets \emptyset$
		\FORALL {$a_r \in a_{rem}$}
		\FORALL {$a_a \in a_{add}$}
			\IF {$equivalent(a_r,a_a)$}
				\STATE $related \gets related \cup \{a_r,a_a\}$
			\ENDIF
			\IF {$seeds(a_r,a_a)$}
				\STATE $related \gets related \cup \{a_r,a_a\}$
			\ENDIF
		\ENDFOR
		\ENDFOR
		\STATE $a_{rem} \gets a_{rem} - related$ 
		\STATE $a_{add} \gets a_{add} - related$		
		\FORALL {$a_r \in a_{rem}$}
		\FORALL {$a_a \in a_{add}$}
			\STATE $\textsc{score}(a_r,a_a) = \textsc{score}(a_r,a_a) + 1$
			\STATE $\textsc{groups}(a_r,a_a) = \textsc{groups}(a_r,a_a) \cup groupId(artf).$
	  \ENDFOR
	\ENDFOR
\ENDFOR
\ENDFOR
\end{algorithmic}
\caption{Migration rule score generation}
\label{fig:switchingAlgo}
\end{figure}

The algorithm exposed in Figure \ref{fig:switchingAlgo} summaries the overall rules extraction process using this filter.

\subsubsection{Post-computation}


We decided to gather artifacts involved in the rules stored in \textsc{SCORE} map based on their \emph{artifactId} property. This choice is justified by the existence of the same artifact under several \emph{groupId}. For example, the \textsc{hsqldb} library can be found under both \emph{groupId}  \texttt{\{"hsqldb"\}} and \texttt{\{"org.hsqldb"\}}. Consequently, we discard the \emph{groupId} of the \emph{migration} rules elements, and merge identical sources and targets parts of the rules. This process is detailed in Table \ref{tab:merge}.

\begin{table}
\centering
\scriptsize{
\begin{tabular}{llllll}

\toprule
\multicolumn{3}{c}{Initial rules}  & \multicolumn{3}{c}{After Merging}  \\
\cmidrule(r){1-3} \cmidrule(r){4-6}
\multicolumn{2}{c}{Rules} & Score & \multicolumn{2}{c}{Rules} & Score \\
\cmidrule(r){1-2} \cmidrule(r){4-5}
org.hsqldb:hsqldb & org.h2database:h2 & 4  & hsqldb &h2 & 5  \\
hsqldb:hsqldb & org.h2database:h2 &  1   & h2 & hsqldb & 7  \\
org.h2database:h2 &hsqldb:hsqldb & 2  & & & \\
org.h2database:h2 &org.hsqldb:hsqldb & 5    & & & \\
\bottomrule
\end{tabular} 
}
\caption{An example of rule merging}
\label{tab:merge}
\end{table}


To improve precision of our technique and to avoid as much as possible false positives, we proceed to a filtering step. The goal of our algorithm is to identify \emph{migration} rules with a reasonable confidence threshold. We determine arbitrarily two conditions that must satisfy a rule $(s,t)$ o be kept as candidates :
\begin{itemize}
\item The \textsc{score} value is $\geq$ 4 and its \textsc{groups} value is $\geq$ 2. 
\item For both $(s,t)$ and $(t,s)$, the \textsc{score} value is $\geq$ 2 and its \textsc{groups} value is $\geq$ 2. 
\end{itemize} 

Each of the popular migration rule needs to be checked manually to make sure the two APIs have the same purpose. This is an important point since it evaluates the precision of our approach.

\subsection{Semi-automatic approach}

The purpose of our approach is to supply recommendation to developers during the software maintenance phase. We obviously attempt to propose correct suggestions. Though, our technique of score lacks precision as false positives rules coexist with true rules. We justify the need to manually assign a binary value whenever a \emph{migration} is true or false. This leads to a creation of base of facts that are definitively either true or false. The correct rules represent the \textsl{seeds} while the wrong are referenced as \textsl{banned}.

This process will be useful in future execution of our tool to observe recent migration trends. Indeed, all the positive rules are loaded at the beginning of the algorithm process. Then, we remove source and target $s$ and $t$ from the sets $a_{rem}$ and $a_{add}$ if the rule $(s,t)$ belongs to \textsl{seeds}. Lines 13-15 in Figure \ref{fig:switchingAlgo} describes this operation. 

When new rules are discovered, we try to automatically assign a correctness value to the rule. To that purpose, we employ the \textsf{seeds} rules to build a \emph{migration} undirected graph \textsf{GM} where nodes $s$ and $t$ are linked if a \textsf{seed} $(s,t)$ exists. Also, a directed graph \textsf{GMB} maintains the wrong migration rules observed until now. 
Graph \textsf{GM} is composed of connected components that represent \emph{categories} of artefacts. We refer as $\textsf{GM}_s$ the connected component that contain the vertex $s$.  
We are capable of giving a correctness score for a rule $(s,t)$ in two situations : 
\begin{itemize}
	\item Score 1 : $t$ $\epsilon$ \textsf{$GM_s$}. Ex : (\textsc{h2},\textsc{hsqldb}), (\textsc{h2},\textsc{derby})$\epsilon$ \textsf{seeds} $\Longrightarrow$ (\textsc{hsqldb},\textsc{Derby}) $\epsilon$ \textsf{seeds}.
	\item Score 0 : $x$ $\epsilon$ \textsf{$GM_s$}, and a path $(x,x_1...x_n,t)$ $\epsilon$ \textsf{GMB}. Ex : \textsc{Derby} $\epsilon$ \textsf{$GM_{H2}$} $\wedge$ (\textsc{Derby},\textsc{Log4J}) $\epsilon$ \textsf{banned} $\Longrightarrow$ (\textsc{H2s},\textsc{Log4J}) $\epsilon$ \textsf{banned}.
\end{itemize} 

Otherwise, the rule requires a manual analysis so that a correctness value can be settled. Finally, the new rules are appended to the \textsf{seeds} or \textsf{banned} base. After an update of the Maven Central Repository, new \emph{migration} rules can be mined using those two bases. Incomplete rules will be manually completed and stored.


\subsection{Mining Usage Trend}

To perform cross-comparison of usage trend on a set of similar APIs $SA$, the history of each artifact of the Maven repository has to be queried.  The purpose is to detect which artifacts  $a \epsilon A$ depend on any artifact $s \epsilon SA$. The structure of the operation-based model allows for such query. The temporal element on the model serves at associating any dependency adoption or resignation with a position in time. Hence, we can evaluate the evolution of the popularity of any given set of similar APIs.  

This cross-comparison provides a deeper insight on the rules generated in the previous step. We propose to plot usage trends of cross-libraries. This enhances APIs popularity increasing or decreasing. Also, if we restrict the usage trend on the number of distinct \emph{groupId} rather than number of artifacts may give another point of view. Indeed, this discards superficial popularity gain when an artifact $a \epsilon A$ produces a new release while keeping the same dependencies. We can assume that the artifacts produced by \textsc{Apache} will keep using their own APIs, like \textsc{Derby} is they need database facilities.




==> study.tex <==
\section{Case study : Maven Central Repository}
\label{sec:study}

For practical reasons, we have realized our case study on projects managed under Maven because 1) it has a centralized repository system of almost 40 000 projects 2) there is a web-based REST API enabling to easily retrieve information from this repository. 

\subsection{Extracting dependencies from Maven}

Maven is a build and dependencies management system for Java software projects. Each project managed by Maven requires a so-called POM (Project Object Model) XML file that contains three mandatory tags: a \textit{groupId} that defines the group owning the project, an \textit{artifactId} that is the unique name of the project under the \textit{groupId}, and a \textit{version} number. POM file also contains a \textit{dependencies} tag where a set of dependencies can be specified, each one by the \textit{groupId} of the dependency, its \textit{artifactId} and optionally its \textit{version}. \figref{pom_model} shows an excerpt of the POM file of \texttt{JUnit} in its \textit{4.10} version.

Project dependencies are stored on a Maven repository. These dependencies are Maven projects as well, and have therefore a POM file as well. The Maven Central Repository\footnote{\url{http://search.maven.org/}} (MCR) is the official Maven repository. It serves over 70 millions downloads every week\footnote{\url{http://www.sonatype.com/people/2010/12/now-available-central-download-statistics-for-oss-projects/}}. It is a relevant data source for our case study for two reasons: 1) the set of projects located on the MCR is large and 2) the dependencies are specified with consistency and can be easily retrieved across projects, which allows us to concentrate on extracting the migration rules.

We now detail how we instantiate our model from the data present on the MCR.  First of all, $P$ is the set of projects located on the MCR. A project $p \in P$ is identified as an element \textit{groupId:artifactId} according to the tags included in its POM file. Each project $p$ has  an associated set $R_p$ containing all its versions. This set is ordered using the versioning scheme used by Maven\footnote{\url{http://docs.codehaus.org/display/MAVEN/Versioning}} applied on the  tag. To obtain a list of dependencies  $d(r), r \in R_p$, we investigate the \textit{dependencies} section of the POM file. It contains several \textit{dependency} tags, from which we extract the \textit{groupId} and \textit{artifactId} tags. This process is illustrated in \figref{pom_model}.

\begin{figure}
  \centering
\includegraphics[width=0.95\linewidth]{pics/pom_model.pdf}
\caption{An excerpt of \textsc{JUnit 4.10} POM file}
\label{fig:pom_model}
\end{figure}

\subsection{Filters to improve rule generation}

Within Maven, a same project can exist under several identities, whereas it should be perceived as a unique one. For example, one project can make use of either \texttt{junit} or \texttt{junit-dep}, with both referring to the \texttt{junit} project. In our opinion, if a project updates its dependency \texttt{junit} to \texttt{junit-dep}, it is not relevant to consider this as a migration rule. Also, the project \texttt{hsqldb} can be found under both \textit{groupId} \texttt{org.hsqldb} and \texttt{hsqldb}. If a project decides to change only the \textit{groupId} of a dependency, we should not consider it as a migration. This situation can lead to the case where two different rules exist but with a similar semantic. For example, (\texttt{org.hsqldb:hsqldb,com.h2database:h2)} and \texttt{(hsqldb:hsqldb,com.h2database:h2)} should be merged as a unique rule. 

To tackle these issues, we propose a four-step process to finally produce migration rule : 
\begin{enumerate}
\item 
We apply a post-processing step after the computation of the sets $\rem(r_i)$ and $\add(r_i)$. Its objective is to remove from these sets the projects that fall into the previous situations.  Our solution is to consider only the \textit{artifactId} of the projects from  $\rem(r_i)$ and $\add(r_i)$,  regardless the \textit{groupId}. 

\item For each element $p$ that both belongs to $\rem(r_i)$ and  $\add(r_i)$, we remove $p$ from those two sets. From now, projects dependencies are only seen with their \textit{artifactId}.

\item We detect the similar remaining elements from these two sets that must be discarded from the analysis. To that purpose, we compute $T_p$ the set of tokens appearing in the \textit{artifactId} of a project $p$. For instance $T_p =$ \{\texttt{junit},\texttt{dep}\} for \textit{junit-dep}. The segmentation is done using non-alphanumeric characters and CamelCase. Then $p$ and $p'$ are removed from resp. $\rem(r_i)$ and $\add(r_i)$ iff $p \in \rem(r_i)$ and $p' \in \add(r_i)$ with $T_p \cap T_{p'} \neq \emptyset$.

\item The Cartesian product can now compute the migration rules. 

\end{enumerate}

An example of this straightforward process is detailed in Figure \ref{filtermaven}. This example highlights the removal of misleading migration rules. For instance, thanks to our process, the rule \texttt{(junit:junit-dep)} is not returned.

\begin{figure*}
\centering
\includegraphics[width=0.95\linewidth]{pics/maven_filter.pdf}
\caption{Maven-specific filter to improve rule generation. From two sets of 3 dependencies, only one rule is kept after the cartesian product.}
\label{filtermaven}
\end{figure*}

As a last point, we introduce $|g(m)|$ as the set of distinct \textit{groupIds} of projects on which $m \in M$ has been observed. This value intervenes as it may happen that several sub-projects within a similar \textit{groupId} perform the same migration. This can be due to a lack of modularity in the project organization. It results that, if a migration rule is observed in 10 sub-projects  simultaneously, its score is increased of 10 as well. However, we think that such situation bias the actual score of a migration rule. We therefore decide to compute the value $|g(m)|$ since it is a better indicator than $|r(m)|$ to estimate the popularity of a migration rule. For instance if $r(m) = \{\mathtt{g_1{:}a_1},\mathtt{g_1{:}b_2},\mathtt{g_2{:}c_1}\}$, $g(m) = \{\mathtt{g_1},\mathtt{g_2}\}$. In the remainder of  the article, we use $|g(m)|$ instead of $|r(m)|$ to evaluate the popularity of a migration rule.
 
\subsection{Results}

The MCR provides a Web REST API to ease the access to the projects it contains. We have used this API to set-up an automatic process and to collect $38588$ projects and $310571$ projects releases. Looking for every $p \in P$ and their associated $R_p$ on the repository took about 2 hours. Mining every associated POM file takes about 35 hours. Computing the rules from every successive couple of set of dependencies {$d(r1),d(r2)$} takes 2 minutes. Before filtering, we obtain a list of $925$ migration rules that constitute the set $M$. 

Among the generated 925 rules,  we need to filter the incorrect rules as much as possible to reduce the manual work when building the expert rules $E$ that we finally deliver. To that purpose, we first use the previously introduced $g(m)$. We include in $E$ only rules having a value $|g(m)|$ $\geq$ 2. The idea behind this statement is that a migration rule gains confidence if it has been observed on several unrelated projects, here at least 2. This filter builds a subset $M' \in M$ of 385 rules.

We decide to retain only rules that have a sufficient confidence value \textit{conf(m)}. We therefore introduce a threshold of confidence value $t_c$ that must be fixed. In order to optimize the threshold $t_c$, we run our tool against the previously computed set $M'$ with different values for $t_c$. Then we manually rate the migration rules found, either as correct or wrong. We aim at maximizing the number of true positives while reducing as much as possible the number of false positives. Results are reported in \figref{minconf}. Note that manually reviewing a rule is usually an easy task as it only requires to look at the websites of the projects to see if they target the same domain. Nevertheless, it is possible that a few false positive were not removed due to a misunderstanding of the libraries features. The whole task of removing the false positives took about 2 hours for rating the 385 rules.

\begin{figure}
\includegraphics[width=0.95\linewidth]{pics/minconf.pdf}	
\caption{Precision evaluation on $t_c$ variations}
\label{fig:minconf}
\end{figure}

According to the results reported in \figref{minconf}, we choose to set $t_c$ to $0.06$ so that we achieve a precision of $0.67$, containing $57$ correct rules and $27$ incorrect rules. Using the $57$ correct rules, we apply the rule augmentation technique described in \alref{augrules}. This technique managed to extend $E$ from $57$ to $80$ rules. This set of $80$ rules is the definitive set of expert migration rules $E$. \tabref{results} shows the $15$ most observed migrations. The whole set $E$ is available online\footnote{\url{http://www.labri.fr/perso/cteyton/index.php?page\_name=rules}}.

\begin{table}
\centering
\footnotesize
\begin{tabular}{llr}
\toprule
\multicolumn{2}{c}{Rule} \\
\cmidrule(r){1-2} Source & Target & $|g(m)|$\\
\midrule
\texttt{commons-logging} & \texttt{slf4j-api} & \texttt{44} \\
\texttt{commons-logging} & \texttt{slf4j-log4j12} & \texttt{21} \\
\texttt{junit} & \texttt{testng} & \texttt{20} \\
\texttt{google-collections} & \texttt{guava} & \texttt{16} \\
\texttt{servletapi} & \texttt{servlet-api} & \texttt{13} \\
\texttt{testng} & \texttt{junit} & \texttt{13} \\
\texttt{slf4j-log4j12} & \texttt{logback-classic} & \texttt{13} \\
\texttt{log4j} & \texttt{slf4j-api} & \texttt{11} \\
\texttt{log4j} & \texttt{logback-classic} & \texttt{11} \\
\texttt{xbean} & \texttt{xmlbeans} & \texttt{10} \\
\texttt{commons-logging} & \texttt{slf4j-simple} & \texttt{8} \\
\texttt{hsqldb} & \texttt{h2} & \texttt{6} \\
\texttt{gfprobe-provider-client} & \texttt{management-api} & \texttt{6} \\
\texttt{commons-logging} & \texttt{log4j} & \texttt{5} \\
\texttt{js} & \texttt{rhino} & \texttt{5} \\
\texttt{xmlParserAPIs} & \texttt{xml-apis} & \texttt{5} \\

\bottomrule
\end{tabular}
\caption{The $15$ most observed migrations from $E$}
\label{tab:results}
\end{table}

Computing the rule association graph leads to $34$ connected components which means that we found $34$ categories. 

\subsection{Valuable information from commits logs}

As stated previously, we had to manually assign as either correct or wrong each migration rule found. Basically, one can search quickly over the internet the validity of the migration. But we consider that the developers are also willing to check the reasons why developers previously performed a migration. In a second time, they want to obtain additional information that support them to perform a migration.

To that purpose, we chose to mine commits logs of a wide set of Java open source projects. The idea is to look for commit logs that match both the source and the target of a given migration rule. Then, the results expose existing commit logs that explicit the migration and/or an associated justification. We arbitrarily selected from four open-source platforms, 5340 projects from Google Code, 16000 from SourceForge, 12308 from Github and 1063 from Apache. We have collected the commits log of total of 34688 projects, resulting in around 3,9M of commit messages. 

We provide on the web page\footnote{\url{http://www.labri.fr/perso/cteyton/search.php}} a search engine that returns a list of commits that can be relevant for the recommendation. To show that this tool can provide assistance for developers when they deal with migration rules, we explicit in Table \ref{tab:commits} an excerpt of commits of interest for Logging and Database facilities. These migrations are discussed in \secref{validation}.

\begin{table}
\begin{tabular}{|p{8.4cm}|}
\hline
\\
\textbf{Logging} \\
\begin{itemize}
\item "logger api changed from \texttt{sfl4j-log4j} to \texttt{logback-classic}"
\item "change logging system from using \texttt{log4j} directly to using \texttt{commons-logging}"
\item "changed to use \texttt{commons-logging} instead of \texttt{log4j} directly"
\item "moved ordi from \texttt{log4j} to \texttt{slf4j-api} to be more easily embeddable"
\item "replaced \texttt{commons-logging} with \texttt{slf4j-log4j12}" 
\item "say goodbye \texttt{log4j}. welcome  \texttt{slf4j-simple}" 
\item "loggers should be of type \texttt{org.slf4j} not \texttt{logback-classic}"
\end{itemize}  \\
\hline
\\
\textbf{Database} \\
\begin{itemize}
\item "replace \texttt{h2} w/\texttt{hsqldb} 2.0 for now"
\item "changed database from \texttt{mysql} to \texttt{hsqldb} 2"
\item "changed default database from \texttt{mysql} to \texttt{derby}"
\item "use \texttt{derby} instead of \texttt{h2} database"
\item "removed \texttt{derby} in favour of \texttt{hsqldb}"
\item "move sql changes from \texttt{h2} to \texttt{mysql} engine"
\end{itemize} \\
\hline
\end{tabular}
\caption{Commit logs for assistance in rule validation (7 commits log for logging utilities and 6 for database facilities)}
\label{tab:commits}
\end{table}

To make sure about the invalidity of a migration rule, the absence of relevant results in the search engine is a solid argument. However, those messages must be used for indications only. There is no guarantee that a sound migration rule will match necessarily at least one meaningful commit log. The set of projects in the database has been chosen arbitrarily with no assumption about the quality of the registered commit logs. However, users are likely to find at least few results against a true migration rule.


==> validation.tex <==
\section{Exploitation of the results}
\label{sec:validation}


\subsection{Analysis of the migration graphs}

In this section we analyse the migration graphs extracted in \secref{study}, and discuss the results we obtained regarding library migration. We compare the conclusion drawn from the graphs with the one that could be drawn from the plot of the evolution of the use of the libraries (this information is computed from the MCR). We show that our migration graphs offer an interesting complement of information and allow to detect interesting libraries which do not really stand out from the evolution plots. Then, we detail four visual patterns that help reading our migration graphs.

For sake of place, we present the analysis of five migration graphs attached to three domains : logging, database and XML. Those categories appear to be among the most utility libraries used in software projects. We have used \textit{JUNG}\footnote{http://jung.sourceforge.net/} to draw them. As explained in \secref{study}, we used $|g(m)|$ instead of $|r(m)|$ to label the arcs. Moreover, in the figures the size of the arcs is proportional to $|g(m)|$. Finally, the number of users of a library is indicated using the color of its node. A dark node indicates that the library is heavily used while a white node indicates that it has only few users. This number of users is relative to the library uses of a category, and is not related to the total number of projects we study.

\subsubsection{Logging}

%\figref{graph_log} shows a migration graph of libraries targeting the logging domain, containing $9$ libraries. We can notice that a significant number of migrations go from \textit{Commons-logging}\footnote{\url{http://commons.apache.org/logging/}}  (80 departures) and \textit{Log4J}\footnote{\url{http://logging.apache.org/log4j/}}(34). Inversely, the library \textit{SLF4J}\footnote{\url{http://www.slf4j.org/}} appears to be a leader and is the target of a high number of migrations. This is even more significant considering that \textit{SLF4J} library is declined in several sub-libraries that appear in the graph with different nodes (e.g., \textit{slf4j-simple}). Also, by computing the score of its respective ingoing edges, it turns out that $30$ \textit{groupIds} have migrated to \textit{LOGBack}\footnote{\url{http://logback.qos.ch/}} and only $2$ times from, targeting \textit{SLF4J}. This may be an indication that projects that migrate to \textit{LOGBack} are globally satisfied. Using this graph, we could recommend to the developers to consider dropping the \textit{Commons-logging} and \textit{Log4J} libraries, and to replace them by \textit{SLF4J} or \textit{LOGBack}. On the web pages of these two libraries we can read ``\textit{The logback-classic module can be assimilated to a significantly improved version of log4j}'' and ``\textit{The Simple Logging Facade for Java or (SLF4J) serves as a simple facade or abstraction for various logging frameworks, e.g. java.util.logging, log4j and logback, allowing the end user to plug in the desired logging framework at deployment time}``. It clearly seems that they aim to replace logging libraries such as \textit{Commons-logging} and \textit{Log4J}.%

\figref{graph_log} shows a migration graph of libraries targeting the logging domain, containing $9$ libraries. We can notice that a significant number of migrations go from \textit{Commons-logging}(80 departures) and \textit{Log4J}(34). Inversely, the library \textit{SLF4J} appears to be a leader and is the target of a high number of migrations. This is even more significant considering that \textit{SLF4J} library is declined in several sub-libraries that appear in the graph with different nodes (e.g., \textit{slf4j-simple}). Also, by computing the score of its respective ingoing edges, it turns out that $30$ \textit{groupIds} have migrated to \textit{LOGBack} and only $2$ times from, targeting \textit{SLF4J}. This may be an indication that projects that migrate to \textit{LOGBack} are globally satisfied. Using this graph, we could recommend to the developers to consider dropping the \textit{Commons-logging} and \textit{Log4J} libraries, and to replace them by \textit{SLF4J} or \textit{LOGBack}. On the web pages of these two libraries we can read ``\textit{The logback-classic module can be assimilated to a significantly improved version of log4j}'' and ``\textit{The Simple Logging Facade for Java or (SLF4J) serves as a simple facade or abstraction for various logging frameworks, e.g. java.util.logging, log4j and logback, allowing the end user to plug in the desired logging framework at deployment time}``. It clearly seems that they aim to replace logging libraries such as \textit{Commons-logging} and \textit{Log4J}.

\begin{figure}
\centering
\includegraphics[width=0.93\linewidth]{pics/graph_loggers.pdf}
\caption{Migration graphs for Logging libraries}
\label{fig:graph_log}
\end{figure}

\figref{all_log} shows the evolution of the use of the four most-used logging libraries. In this figure, we can notice that \textit{SLF4J} stands out from the other ones, which strengthens the conclusion drawn from the migration graph. However, \textit{LOGBack} does not appear as particularly interesting and would probably not be seriously considered using only this plot.

\begin{figure}
\includegraphics[width=0.98\linewidth]{pics/loggers.pdf}
\caption{Evolution of the use of the logging libraries}
\label{fig:all_log}
\end{figure}

\subsubsection{Database}

%Within the database category, we observe several balanced migrations between \textit{HSQLDB}\footnote{\url{http://hsqldb.org/}}, \textit{Derby}\footnote{\url{http://db.apache.org/derby/}}, and \textit{MySQL}\footnote{\url{http://www.mysql.com/}}. We also notice that $6$ \textit{groupIds} have migrated from \textit{HSQLDB} to \textit{H2}\footnote{\url{http://www.h2database.com/html/main.html}}, and nobody did migrate from \textit{H2}. By looking to this graph, we could recommend to the projects to seriously consider using \textit{H2}. By looking on the web page of \textit{H2}, it seems that it has more features\footnote{\url{http://www.h2database.com/html/features.html}} than its competitors, and very good performances\footnote{\url{http://www.h2database.com/html/performance.html}}. Interestingly, we did perform a migration from \textit{HSQLDB} to \textit{H2} in one of our own software projects\footnote{\url{http://harmony.googlecode.com}} when seeing these figures, with a significant gain in features and performances.%

Within the database category, we observe several balanced migrations between \textit{HSQLDB}, \textit{Derby}, and \textit{MySQL}. We also notice that $6$ \textit{groupIds} have migrated from \textit{HSQLDB} to \textit{H2}, and nobody did migrate from \textit{H2}. By looking to this graph, we could recommend to the projects to seriously consider using \textit{H2}. By looking on the web page of \textit{H2}, it seems that it has more features than its competitors, and very good performances. Interestingly, we did perform a migration from \textit{HSQLDB} to \textit{H2} in one of our own software projects\ced{Harmony} when seeing these figures, with a significant gain in features and performances.

\begin{figure}
\centering
\includegraphics[width=0.85\linewidth]{pics/graph_db.pdf}
\caption{Migration graph for the database libraries}
\label{fig:graph_db}
\end{figure}%

In contradiction to our approach, \figref{all_db} presents a classic evolution of the use of the database libraries. We can observe that \textit{MySQL} interest is a bit slowing down, and that \textit{HSQLDB} stands as the leader. Using only this plot, the \textit{H2} library would not arise as interesting since it has less users than its competitors.

\begin{figure}
\includegraphics[width=0.98\linewidth]{pics/dbs.pdf}
\caption{Evolution of the use of the database libraries}
\label{fig:all_db}
\end{figure}

\subsubsection{XML}

%\figref{graph_xmls} shows the three migration graphs that can be attached to the XML domain. \textit{XMLBeans}\footnote{\url{http://xmlbeans.apache.org/}} looks like an emerging library as it underwent a migration from within $10$ distinct \textit{groupIds}. It seems to be the preferred target of the users of \textit{XBeans}\footnote{\url{http://www.xbeans.org/}}. By looking to their websites, we did not understand the reason for this migration, although we have evidence in the SVN commit logs that it is not a false positive. \textit{xml-apis} is preferred to \textit{xmlParsersAPI}. By looking in the Maven repository, we noticed that in fact it is the same library, that was not eliminated by our text-mining techniques. Nevertheless, \textit{xmlParsersAPI} is the outdated one. Finally, \textit{SJSXP} and \textit{Woodstox}\footnote{\url{http://woodstox.codehaus.org/}} (wstx) are two STAX-compliant XML processors. As there are few users of \textit{SJSXP}, and as some of them are migrating to \textit{Woodstox}, the later seems to be the library of choice in for STAX compliant parsers. This intuition is strengthened when looking at \figref{stax_use}, which shows that \textit{wstx} is the largest used STAX-compliant XML found with our migration rules.% 

\figref{graph_xmls} shows the three migration graphs that can be attached to the XML domain. \textit{XMLBeans} looks like an emerging library as it underwent a migration from within $10$ distinct \textit{groupIds}. It seems to be the preferred target of the users of \textit{XBeans}. By looking to their websites, we did not understand the reason for this migration, although we have evidence in the SVN commit logs that it is not a false positive. \textit{xml-apis} is preferred to \textit{xmlParsersAPI}. By looking in the Maven repository, we noticed that in fact it is the same library, that was not eliminated by our text-mining techniques. Nevertheless, \textit{xmlParsersAPI} is the outdated one. Finally, \textit{SJSXP} and \textit{Woodstox} (wstx) are two STAX-compliant XML processors. As there are few users of \textit{SJSXP}, and as some of them are migrating to \textit{Woodstox}, the later seems to be the library of choice in for STAX compliant parsers. This intuition is strengthened when looking at \figref{stax_use}, which shows that \textit{wstx} is the largest used STAX-compliant XML found with our migration rules. 

\begin{figure}
\centering
\includegraphics[width=0.87\linewidth]{pics/graphs_xmls.pdf}
\caption{Migration graph of the three XML categories}
\label{fig:graph_xmls}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=0.87\linewidth]{pics/stax_use.pdf}
\caption{Evolution of the use of stax-compliants libraries}
\label{fig:stax_use}
\end{figure}


\subsection{Visual Patterns}

To assist the analysis of a migration graph, we propose four visual patterns that can be quickly observed. These patterns allow to characterize some specific migrations. First, the \textit{Gold Rush} pattern is observed when a library has many input migrations and few output ones. This clearly means that many projects migrate to this one. We believe this library has certainly more advantages than the other ones. As a consequence, the \textit{Gold Rush} pattern can be used as a choice criteria to choose the right library to migrate to. On the contrary, we would not recommend projects that match the target of the \textit{exodus} pattern, such as \textit{commons-logging}. The \textit{Pong} pattern refers to a bi-directional migration, that does not promote a project more than an other. The \textit{Challenger} denotes a recent but promising candidate, as it has been adopted widely in a short period of time.

\tabref{patterns} briefly summarizes these patterns. For each pattern, it explains how to observe the pattern, and provides an advice for developers that think about migrating their libraries.

\begin{table*}
\centering
\begin{tabular}{p{2.2cm}p{1cm}p{8cm}p{3cm}}
\toprule
\textsc{Name} & \textsc{Target} & \textsc{Description} & \textsc{Example} \\
\midrule
\textbf{Gold Rush} & Library & A library has many input migrations and few output ones. Developers should consider migrating to it. & \textsc{slf4j-api} \\
\hline
\textbf{Exodus} & Library & A library has many output migrations and few input ones. Developers should consider to stop using it. & \textsc{commons-logging} \\
\hline
\textbf{Challenger}  & Library & A library that is the target of a significant number of migrations originating from the most used library. Developers should consider migrating to it. & \textsc{H2} \\
\hline
\textbf{Pong} & Migration & Bi-directional migration rules with similar occurrences, no conclusion can be drawn from this pattern. & (\textsc{hsqldb},\textsc{derby}) \\
\bottomrule
\end{tabular}
\caption{Visual patterns observed in the migration graphs}
\label{tab:patterns}
\end{table*}


==> validation_oss.tex <==
\section{Exploitation of the results}
\label{sec:validation}

This section answers the research questions presented in \secref{intro} by presenting the results of our study. 

\subsection{In which projects migrations are performed?}

As described in the Section \ref{sec:approach}, we removed from the corpus the projects judged irrelevant for this analysis. 8600 projects remained after this operation. \tabref{deciles} presents the decile of the three metrics (KLOC, Commit, Duration) we choose to measure on these projects. For each metric, we used these deciles to compute groups of quite similar projects.

\begin{table}[h]
\centering
\small{
\begin{tabular}{lcccccccccc}
\toprule
Group & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule
\textbf{Java KLOC} & 0.54 & 0.96 & 1.5 & 2.2 & 3.2 & 4.9 & 7.7 & 13.7 & 30.4 & 3675\\
\midrule
\textbf{Commit} & 25 & 31 & 38 & 49 & 65 & 87 & 127 &  207 & 430 & 29656 \\
\midrule
\textbf{Duration} & 3 & 5 & 6 & 8 & 11 & 15 & 21 & 29 & 45 & 512 \\
\bottomrule
\end{tabular}
}
\caption{Upper bound values for the 30 deciles formed using CLOC, Commit and Duration distributions}
\label{tab:deciles}
\end{table}

We then compute the number of migrations for each group and for each metrics. Tables \ref{tab:group_kloc}, \ref{tab:group_commit} and \ref{tab:group_kloc} present the groups for each metrics and present how many projects are contained in each group and how many migrations have been performed.


\begin{table}[h]
\centering
\footnotesize{
\begin{tabular}{lcccccccccc}
\toprule
Group & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule
\textbf{Java KLOC} &  & $>$ 0.54 & $>$ 0.96 & $>$  1.5 & $>$  2.2 & $>$  3.2 & $>$  4.9 & $>$  7.7 & $>$  13.7 & $>$  30.4  \\ 
 & $\leq$ 0.54 & $\leq$ 0.96 & $\leq$ 1.5 & $\leq$ 2.2 & $\leq$ 3.2 & $\leq$ 4.9 & $\leq$ 7.7 & $\leq$ 13.7 & $\leq$ 30.4 & $\leq$ 3675\\
\midrule
\textbf{Projects} & 851 & 850 & 843 & 838 & 831 & 837 & 838 &  814 & 822 & 812 \\
\midrule
\textbf{Migrations} & 6 & 13 & 17 & 22 & 29 & 22 & 23 & 46 & 38 & 47 \\
\bottomrule
\end{tabular}
}
\caption{The groups for the KLOC metrics}
\label{tab:group_kloc}
\end{table}


\begin{table}[h]
\centering
\footnotesize{
\begin{tabular}{lcccccccccc}
\toprule
Group & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule
\textbf{Commit} &  & $>$ 25 & $>$ 31 & $>$ 38 & $>$ 49 & $>$ 65 & $>$ 87 & $>$ 127 &  $>$ 207 & $>$ 430 \\ 
 & $\leq$ 25 & $\leq$ 31 & $\leq$ 38 & $\leq$ 49 & $\leq$ 65 & $\leq$ 87 & $\leq$ 127 & $\leq$ 207 & $\leq$ 430 & $\leq$ 29656 \\
\midrule
\textbf{Projects} & 840 & 869 & 791 & 857 & 900 & 829 & 833 & 825 & 815 & 777 \\
\midrule
\textbf{Migrations} & 0 & 3 & 7 & 12 & 18 & 22 & 29 & 40 & 46 & 86 \\
\bottomrule
\end{tabular}
}
\caption{The groups for the Commit metric}
\label{tab:group_commit}
\end{table}


\begin{table}[h]
\centering
\footnotesize{
\begin{tabular}{lcccccccccc}
\toprule
Group & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule
\textbf{Duration} &  & $>$ 3 & $>$ 5 & $>$ 6 & $>$ 8 & $>$ 11 & $>$ 15 & $>$ 21 & $>$ 29 & $>$ 45  \\ 
 & $\leq$ 3 & $\leq$ 5 & $\leq$ 6 & $\leq$ 8 & $\leq$ 11 & $\leq$ 15 & $\leq$ 21 & $\leq$ 29 & $\leq$ 45 & $\leq$ 512 \\
\midrule
\textbf{Projects} & 704 & 749 & 769 & 918 & 872 & 892 & 949 &  839 & 838 & 806 \\
\midrule
\textbf{Migrations} & 4 & 4 & 5 & 10 & 17 & 33 & 27 & 52 & 45 & 66 \\
\bottomrule
\end{tabular}
}
\caption{The groups for the Duration metrics}
\label{tab:group_duration}
\end{table}

To evaluate if the number of migrations was independent of the group, we used statistical Chi-squared test. The null hypothesis is that the proportion of migrations is the same whatever the group for each metrics. This test was therefore computed for the three metrics. \tabref{deciles} presents the results of the chi-squared test. We observe that our corpus is significant and that the null hypothesis is rejected with a probability of $5\%$. This means that the proportion of migrations is not the same depending of the group for each metric.

\begin{table}[h]
\centering
\begin{tabular}{lccc}
\toprule
& CLOC & Commit & Duration \\
\midrule
X-square & 66.1 & 235.0 & 158.9 \\
degree of freedom & 9 & 9 & 9 \\
p-value & $8.8*10^{-11}$ & $2.2*10^{-16}$ & $2.2*10^{-16}$ \\
\bottomrule
\end{tabular}
\caption{Results for the chi-square test}
\label{tab:deciles}
\end{table}

To visualize the differences in proportion of each group, we plot in \figref{ratio} the ratio (number of migration per number of projects) for each metric. This Figure clearly shows that the proportion of migrations is more important in the biggest projects (in terms of KLOC, duration and commit). However, the increase of the values is still slow. The highest ratio is featured by the Commit metric. In that case, 11\% of the projects that have more than 430 commits have performed at least one migration.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{pics/jsep/ratio.pdf}
\caption{Distribution of migrant projects per CLOC, Commit and Duration deciles}
\label{fig:ratio}
\end{figure}

These results give interesting information to answer our first research question. First of all, it is clear that few projects perform library migrations. Second, mature projects (in terms of KLOC, Commit and duration) have a higher probability to perform at least one migration. Finally, the number of commit and the duration are much more relevant to measure the maturity of a project than the KLOC for our concern. Furthermore, our results clearly show that almost 10\% of the projects that have a very long duration or a large number of commits perform migrations. 



\subsection{Which libraries are migrated?}

By grouping the 134 migrations rules we identified in our study, we obtained 38 library categories. %The Figures \ref{fig:logging_graph} and \ref{fig:graph_json} present the graphs that correspond to the Logging and JSON categories. The migration graphs from the remaining categories are available online\ced{TODO}. We recall that a migration graph presents a category of similar libraries and highlights the migrations that have been performed between them (cf. Section \ref{sec:approach}).
\figref{categories} presents how migrations are distributed among these library categories. For the sake of readability, we restrain this chart to the 20 categories that have at least 2 migrations. We observe that the first 6 categories contain 74\% of the migrations, and the first 8 and 16 cover respectively 85\% and 95\% of the migrations. This result gives a first partial answer to our research question since those libraries are prone to migration. 

%The nine first categories contain 83\% of all the identified migrations (\textsl{logging}, \textsl{testing}, \textsl{json}, \textsl{http}, \textsl{database}, \textsl{collections}, \textsl{test-utlis} and \textsl{xml}). 




\begin{figure}[h]
\centering
\includegraphics[width=0.67\linewidth]{pics/jsep/categories.pdf}
\caption{Distribution of migrations between the categories having at least 2 migrations}
\label{fig:categories}
\end{figure}


The left part of \figref{categories_si} shows the number of library contained within each category. This figure clearly shows that the categories contain few libraries (mean = 4.55). This maybe explains why few projects perform migrations as there are not so many target replacement libraries to migrate to. Further, this figure also shows that the number of migrations per category is not correlated with the number of libraries contained in the category.% The right part of this same figure shows how many projects depend at least on one library of each category. 
 The right part of this same figure shows how many library introductions are counted for each category. Unsurprisingly, the two categories that contains the more migrations contain libraries that are used by the most of projects. Surprisingly, many projects use a \textsl{xml} library but they do not perform a lot of migrations. The reason is because the \textsl{xml} category contains the native Java XML Application Programming Interface, which is used by many projects. 

\begin{figure}[h]
\centering
\includegraphics[width=0.99\linewidth]{pics/jsep/categories_size_intro.pdf}
\caption{Number of library within a graph and number of projects that depend at least of one library of the graph}
\label{fig:categories_si}
\end{figure}


These results give many information to answer our research question. There exists categories of libraries that are prone to migration. We now investigate deeper in the categories to better understand if there exists libraries that are prone to migration. We choose to present the \textsl{logging} category as it is the one that contains most of the migration. We also choose to present the \textsl{json} category as it contains few migrations but contains several libraries.

%: Logging, Testing and JSON. It should be noted that the \textsl{http} category is particular since it contains two rules for which 28 migrations have been performed. These two rules correspond to a popular migration that consists in replacing the \textit{commons-httpclient} library by \textit{httpclient} and \textit{httpcore}. 

%\paragraph{Logging}

\figref{logging_graph} shows the migration graph that includes libraries of the logging domain. We recall that a migration graph presents a category of similar libraries and highlights the migrations that have been performed between them (cf. Section \ref{sec:approach}). The noticeable observation here is the high number of migrations that go to the library \lib{SLF4J} (33+38=71). Moreover, many migrations go from the library \lib{Commons-logging}(33+11=44) and from the library \lib{Log4J} (38+8+6=50). We also note that \lib{LOGBack} is sometimes used to replace \textit{Log4J}, but only this library. Moreover, only 3 projects gave up \lib{SLF4J} in favour of \lib{Log4J}. 
%Looking at the web pages of these two libraries we can read ``\textit{The logback-classic module can be assimilated to a significantly improved version of log4j}'' and ``\textit{The Simple Logging Facade for Java or (SLF4J) serves as a simple facade or abstraction for various logging frameworks, e.g. java.util.logging, log4j and logback, allowing the end user to plug in the desired logging framework at deployment time}``. It clearly seems that they aim to replace logging libraries such as \textit{Commons-logging} and \textit{Log4J}. 

\begin{figure}[h]
\centering
\includegraphics[width=0.50\linewidth]{pics/jsep/jung_loggers.pdf}
\caption{Migration graph for the logging category}
\label{fig:logging_graph}
\end{figure}

\figref{usage_logging} shows the number of projects of our corpus that use a logging library and the evolution of library usage from 2009 to 2013. This Figure first shows that \lib{Log4j}, \lib{Slf4J} and \lib{commons-logging} are the most used libraries in Java software development (3425 projects in our corpus use one of these library). Secondly, the Figure also shows the increase use of these three libraries, particularly for \lib{Slf4J}. Further 1,000 projects use \lib{Slf4J} in 2013. As we know that 71 migrations go to \lib{Slf4J}, this means that about 7\% of the projects that use \lib{Slf4J} were using another logging library before. Moreover, knowing that there are 50 migrations that go from \lib{Log4J}, this means that even if it is currently the most popular library, it is also the most given up one. 

\begin{figure}[h]
\centering
\includegraphics[width=0.60\linewidth]{pics/jsep/usage_loggers.pdf}
\caption{Use evolution of logging libraries}
\label{fig:usage_logging}
\end{figure}

%The logging category represents 97 migrations in our corpus. The total number of logging library introductions is 4221, which represents a ratio $\frac{97}{4221} = 0.02$. This low value means that even in the most active categories in terms of migration, usage of libraries does not necessarily lead to a replacement in most of the cases. 

%\paragraph{JSON}

Figure \ref{fig:graph_json} shows the migration graph that includes libraries of the JSON domain. JSON is a standard for data interchange over Web applications that is commonly and widely used nowadays. The graph contains 9 libraries and shows 30 migrations. The migrations in this graph are rather balanced. The graph shows that \lib{jackson} and \lib{gson} are mainstream alternatives for library replacements. Moreover, it should be noted that \lib{org.json} is the source of 15 of migrations (50\% of the migrations).

%This momentum has been followed by the growth of several libraries capable of handling JSON format. Nine of them are gathered in Figure \ref{fig:graph_json}. The most used among these facilities, which is also the oldest, is \textit{org.json}. However, we can observe a total of 15 outgoing migrations from this library. 

%Note that \textit{xstream} solution is a utility which is not only designed to parse JSON data, but natively processes XML documents. The rest of the libraries are otherwise exclusively JSON-oriented. This category is therefore interesting since it highlights a rich but still not closed set of possible replacements for JSON processors. 

\begin{figure}[h]
\centering
\includegraphics[width=0.90\linewidth]{pics/jsep/jung_json.pdf}
\caption{Migration graph of the JSON category}
\label{fig:graph_json}
\end{figure}

\figref{usage_json} shows the number of projects of our corpus that use a JSON library and the evolution of library use from 2009 to 2013. This figure shows that all libraries except \lib{org.json} are almost used by the same number of projects. \lib{org.json} is the most used library and has a strong increase since 2011.  Moreover, \lib{gson} and \lib{jackson} have also a strong increase since 2012. Knowing that these two libraries are used as target to replace \lib{org.json} they then can be considered to be candidate libraries to migrate to. 

\begin{figure}[h]
\centering
\includegraphics[width=0.75\linewidth]{pics/jsep/usage_json.pdf}
\caption{Evolution of number of client projects the JSON category}
\label{fig:usage_json}
\end{figure}

%The JSON category represents 30 migrations in our corpus. The total number of JSON library introductions is 1631, which represents a ratio $\frac{30}{1631} = 0.018$. It is a bit less than logging libraries but rather similar. The intuition that arise from these observations is that there is no category of libraries that are frequently replaced.

%\paragraph{Testing}
%
%To conclude, we display two distinct categories that we gathered for sake of readability and since they are small-size and are used in the same context of software testing. It includes testing and mocking libraries. The ahead is compounded of the major framworks \textit{JUnit} and \textit{TestNG}, the first one being the indisputable leader in this domain in terms of popularity. The second sub-category gathers elements used during software testing, in particular to simulate object behavior and ease unit testing. The migration graph associated to this category is shown in \figref{test_graph}.
%
%Similar to the observation made in our previous study, the solution \textit{TestNG} seems more and more adopted in favor of \textit{JUnit}, and stands thus as a robust candidate for migration. We did investigate \textit{TestNG} over the web to understand this trend, and it appears to merely offer more functionalities that \textit{JUnit}. Finally, the library \textit{Mockito} is a recognized solution as none project gave it up. The surprising fact is that \textit{JUnit} is significantly more popular than \textit{TestNG}, contrary to the observed trend. We can conclude that the popularity of a library can not indicate its migration activity.
%
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.70\linewidth]{pics/jsep/jung_test.pdf}
%\caption{Migration graph of the Testing utilities}
%\label{fig:test_graph}
%\end{figure}
%
%
%Now, we analyze how much projects use any of these libraries. Results shown in \figref{test_usage} confirm that \textit{JUnit} stays the leader in the domain of Testing for Java Applications, and its popularity is not surprising. The fact that 332 projects only make use of \textit{TestnG} is interesting. It means that 6.32\% of the current \textit{TestNG} users come from \textit{JUnit}, which is a significant number with respect to the overall number of migration founds in our corpus. The chart also confirms the rapid increase of \textit{Mockito} since 2010. It lets also think that \textit{Hamcrest} is a serious reference in this domain. 
%
%\begin{figure}[h]
%\centering
% \begin{subfigure}[b]{0.40\textwidth}
% \centering
%  \includegraphics[width=\textwidth] {pics/jsep/usage_test.pdf}
%  \caption{Test libraries}
%  \label{fig:test_usage}
% \end{subfigure}
% \begin{subfigure}[b]{0.59\textwidth}
% \centering
%  \includegraphics[width=\textwidth] {pics/jsep/usage_mock.pdf}
%  \caption{Test utilities}
%  \label{fig:mock_usage}
%  \end{subfigure}
%  \caption{Usage rate evolution for the Testing category}
%   \label{fig:test_usage}
%\end{figure}
%
%We do not compute the library introductions score in this category since it it too biaised by the impressing popularity of \textit{JUnit}. We can however note that more than 50\% of the projects in the corpus pratice unit testing. The particularity of this category is the lack of existing alternatives to \textit{JUnit}, except \textit{TestNG}. Once again, the ratio of migrations is relatively low in this category.

%\paragraph{Conclusion}

The deep analysis of a category give much more information to answer our research question. There clearly exists libraries that are prone to migration. This depends on the domain as well as the number of existing libraries in the domain. The \textsl{Logging} and the \textsl{json} domains are good illustration to that phenomena. The analysis of the other domains also highlights other libraries that are prone to migration even if few migrations are performed \footnote{http://www.labri.fr/perso/cteyton/index.php?page_name=migrations}. %However, this does not mean that they are easier to replace than other categories of libraries. We argue that the majority of the libraries can be replaced by another solution. The fact that a minority of categories encompasses most of the migrations is mainly due to their higher usage popularity. It is also related to the existence of several competitive solutions it these categories . Our analysis showed that there are no specific categories of libraries that are frequently changed, in a relative point of view from their overall usage. Indeed, even inside the most active ones, the ratio of migrations is relatively low. 


\subsection{When migrations are performed?}

To check if there is any tendency regarding migrations we create a migration-time diagram for each category. For the sake of clarity, we only present in this paper the migration-time diagram of the \textsl{Logging} category. The migration-time diagrams of the other categories are available on line \footnote{http://www.labri.fr/perso/cteyton/index.php?page_name=migrations}.

\figref{time_log} shows the migration-time diagram of the \textsl{Logging} category. This category contains 6 rules that are presented on the y-axis. The diagram clearly shows that some rule are time framed such as the (\lib{log4j} $\rightarrow$ \lib{commons-logging}) one. The other rules exist during all the period shown by the diagram. 

This diagrams also shows how many migrations are performed for each rule. For instance, it shows that the migrations that target \lib{slf4j} have been increasingly performed since 2010. It also shows that the few migrations that target \lib{log4j} are performed time to time since 2005.

%Even if this diagram clearly shows tendency it does not explain them.  graph for the rule \textit{Log4j} $\rightarrow$ \textit{Commons-Logging}. The migration dates range from August 2008 to May 2010. Since this date, no one changed its logging utility to \textit{Commons-Logging}, as shown by the bottom line (\textit{*} $\rightarrow$ \textit{Commons-logging}) which gathers all the adoptions for this library. This migration can be seen as outdated.Inversely, \textit{Log4j} has undergone many departures and the majority happened since 2009 until now in 2013, which means that leaving \textit{Log4J} is a current and active trend. \textit{Logback} adoptions start from late 2009 until 2013, thus choosing this solution is still topical. The significant recent moves to\textit{Slf4J} confirm its current status of leader in migrations.


\begin{figure}[h]
\centering
\includegraphics[width=0.97\linewidth]{pics/jsep/loggers.pdf}
\caption{Migration-time diagram of the \textit{Logging} category}
\label{fig:time_log}
\end{figure}


%\figref{jsontime} exhibits the migrations through time for the rule \textit{org.json} $\rightarrow$ \textit{Gson}. The chart unveils two interesting facts. First, 7 migrations out of 8 target \textit{Gson} between 2012 and 2013, from 3 distinct librairies. It strenghens the recent increase of \textit{Gson} adoptions. Similarly, we enumerate 10 out of 14 migrations that originate from \textit{org.json} that happened after August 2011. It suggest that \textit{org.json} is recently switched for various alternatives, and this may constitute an early sign of exodus. 
%
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.90\linewidth]{pics/jsep/org_gson.pdf}
%\caption{Migrations trends for the rule \textit{org.json} $\rightarrow$ \textit{Gson}}
%\label{fig:jsontime}
%\end{figure}
%
%\paragraph{Testing}
%
%As a last example, attention is paid to the migration \textit{JMock} $\rightarrow$ \textit{Mockito}. \figref{time_mock} learns us that \textit{JMock} has been dropped for 2007 and there is not peak of activity for this library. Inversely, we confirm the recent adoption of \textit{JMockito} which started in late 2008. It is also interesting to notice that 5 out of 6 projects \textit{JMock} have switched to \textit{Mockito} between 2009 and 2011. The last made the move more recently in 2013, which finally strenghtens that this migration is not outdated.
%
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.90\linewidth]{pics/jsep/jmock_mockito.pdf}
%\caption{Migrations trends for the rule \textit{JMock} $\rightarrow$ \textit{Mockito}}
%\label{fig:time_mock}
%\end{figure}
%
%\paragraph{Conclusion}

Migration-time diagrams help to answer our research question as it clearly appears that some migrations are performed during specific period of time. However, these diagrams do not explain why such tendencies are observed. A further analysis of the status of the migrated library as well as the status of the projects that perform the migration should be done to better understand if the period of time as any influence on the performed migrations.

%quickly identify if the existence of key time periods with respect to a migration. The aggregated migrations \textit{(source $\rightarrow$ *)} and \textit{* $\rightarrow$ target} propose a relative view on the situation of the two libraries in their category migration trends. Whereas some migrations are too scattered in time to draw any conclusion, in some cases concentration of migrations in a period of time is noticed. A significant concentration is seen as a "buzz" effect, and may help developers to detect the most recent trends. Such trend can be either a \textit{rush} to or an \textit{exodus} from a library. To complete anwer to \textsc{RQ4}, we advice to integrate the time information for library migrations studies.

\subsection{Why migrations are performed?}

By manually reviewing the commit logs of projects that have migrated we have only found 12 logs that contain the clear motivation of the migration. These logs are exposed in Table \ref{commits_reasons}. The two most reported reasons here are \textsl{Feature} and \textsl{Configuration}.

\begin{table}[h]

\centering
\footnotesize{
\begin{tabular}{lp{7cm}l}
\toprule
\multicolumn{1}{c}{\textbf{Migration}} &\multicolumn{1}{c}{\textbf{Message}} & \multicolumn{1}{c}{\textbf{Reason}} \\[2ex]
\midrule
\textit{commons-logging} $\rightarrow$ \textit{slf4j} & \textit{"replacing commons-logging with slf4j to help with osgi compliance per springsource recommendation."} & Configuration \\
\midrule
\textit{junit} $\rightarrow$ \textit{testng} & \textit{"use testng instead of junit which is a lot more configurable in test selection (and allows us to do a much better job a leaving the tree green even while developing tests that are known to fail)"} & Feature \\
\midrule
\textit{junit} $\rightarrow$ \textit{testng} & \textit{"convert tests to testng because we have groups here"} & Feature \\
\midrule
\textit{log4j} $\rightarrow$ \textit{commons-logging}& \textit{"switched from a log4j based logging api usage to commons-logging in order to allow enhanced logging techniques to be optional} & Feature \\
\midrule
\textit{log4j} $\rightarrow$ \textit{logback} & \textit{"simple migration to logback since log4j is old"} & Outdated \\
\midrule
\textit{log4j} $\rightarrow$ \textit{logback}& \textit{"changed to logback to allow change of log levels"} & Feature \\
\midrule
\textit{org.json} $\rightarrow$ \textit{gson} & \textit{"replaced json.org package with gson for license compatibility"} & License \\
\midrule
\textit{json-lib} $\rightarrow$ \textit{jackson} & \textit{"use jackson json library (reduce dependencies)"}& Configuration \\
\midrule
\textit{json-lib} $\rightarrow$ \textit{org.json}& \textit{"demonstrate bug in json-lib"} & Bug \\
\midrule
\textit{org.json} $\rightarrow$ \textit{json-smart} & \textit{"change org.json library (don't be evil licence) by json smart (apache license 2.0)"} & License \\
\midrule
\textit{commons-collections} $\rightarrow$ \textit{lambadj} & \textit{"replaced commons-collections with lambdaj since it has a more modern search syntax"} & Feature \\
\midrule
\textit{gson} $\rightarrow$ \textit{org.json} & \textit{"attempting to get into maven central repo. requires moving from gson which isn't in central (except buggy version)"} & Configuration \\
\bottomrule
\end{tabular}
}
\caption{Commit logs that justify library migrations}
\label{commits_reasons}
\end{table}

The amount of data collected is not sufficient to propose a significant taxonomy for the motivations. Even if the logs provide rich and interesting information, we cannot infer anything based on so few data. Moreover, we do not know why the logs do not explicitly precise the motivations of the migrations. Section \ref{sec:conclusion} discusses perspectives to better deal with this research question. 


%The 7 arbitrarily categories differ in their nature and are various. For instance, the library \textit{org.json} is under a license which we can qualify as "exotic"\footnote{http://java.dzone.com/articles/jsonorg-license-literally-says}. But for legacy reasons, developers would prefer to use external libraries with a known license. We discovered also a project that change from \textit{json-lib} to \textit{jackson} since the number of transitive dependencies to integrate was less important. This may be a side effect of component reusability in software development. It is interesting to notice that some of the exposed reasons are subtle and certainly ignored from library maintainers. 

%To conclude on \textsc{RQ5}, understanding choices that prevailed to migrate libraries is a richful information that reveals interesting facts about libraries. However, finding this data is a complex operation for the moment. Our attempt with projects commit logs was a feasible starting point, unfortunately they do not contain enough valuable information. This can be explained by the general lack of strictness in developers commit logs quality, since they are not compelled to write commit messages of good quality. We will discuss in Section \ref{sec:fw} the perspectives to investigate and figure out why developers complete library migrations.

\subsection{How migrations are performed?}


To measure the time needed for migrations, we went through the history of all the projects that performed a migration rule. For the 342 migration occurrences identified, we measured the number of commits required, and the number of \textit{commit} days and developers as well. The results in \tabref{lib_mig} presents the distribution of the migrations per values for the three characteristics.

\begin{table}[h]
\centering
-\footnotesize{
\begin{tabular}{lccccccccccc}
\toprule
 & \multicolumn{10}{c}{\textbf{Values}} \\
\cmidrule {2-11}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  $>=$10 & Total \\
\midrule
\# Commits & 79.3 \% & 3.2 \% & 3.4 \% & 0.6 \% & 1.7 \% & 1.7 \% & 1.4 \% & 0.9 \% & 1.1 \% & 6.6 \% & 100 \%   \\
\# Days & 88.0 \% & 3.7 \% & 4.3 \% & 0.6 \% & 0.9 \% & 1.1 \% & 0.3\% & 0.3 \% & 0.0\% & 0.9 \% & 100 \% \\
\# Authors & 94.2 \% & 4.9 \% & 0.6 \% & 0.3 \% & 0 \% & 0 \% & 0 \% & 0 \% & 0 \% & 0 \% & 100 \% \\
\bottomrule
\end{tabular}
}
\caption{Distribution of library migrations per number of commit, commit days and developers  (\# : number of)}
\label{tab:lib_mig}
\end{table}

It shows that 79.3\% of the migrations are achieved within a unique commit. The 20.7 \% remaining are distributed over various values, but it is still interesting to see that 6.6\% of the migrations last more than 10 commits. This number of 20.7 \% affirms that library coexistence is common in practice. The process of transformation mainly happens during one calendar day, as only 12\% of the library cohabitations remains at least 2 days in the project. Finally, a large majority of the work is completed by a unique developer (94.2 \%). 


We manually reviewed commit logs for migrations achieved during at least 2 commits and looked for clues of issues or painful efforts with respect to migrations. Unfortunately, we could not find any data of interest. The only message that expressed some kinds of feelings concerned a migration \lib{velocity} $\rightarrow$ \lib{Freemarker} : \textit{"Hopefully the last issue remaining from the conversion to FreeMarker fixed"}. 

To answer \textsc{RQ5}, library migrations is a process that most of the time is accomplish between two project consecutive versions. However, explaining this practice is far from trivial. In our opinion, it just reveals common development habits. Measuring the efforts and collecting the issues faced by developers were attempted but not successful due to a lack of data.

Finally, this analysis reflects that the distance to choose between two project versions for our approach should not be too small, otherwise some migrations will be missed. Optimizing this value is therefore complex.


%
%For the two logging libraries, all the 19 migrations happened in a pattern $t_{start}$= $t_{end}$, i.e. one single commit was enough to switch from \textit{Log4J} to \textit{Commons-logging} and vice-versa. Some API design similarities must explain that the source code transformations are not a tedious task.
%
%16 out of the 21 projects that changed \textit{JUnit} in favor of \textit{TestNG} achieved the migration in one commit. One project kept \textit{junit} during 6 commits through 5 distinct \textit{commit} days. One another needed 10 commits, 1 person and 5 \textit{commit} days, while a different one spent 9 commits during 1 day with 1 person. The two remaining projects had just respectively 2 and 3 commits to accomplish the migration. Analyzing the commits logs of these projects does not enhance any particular reason for these scenarios. On the 11 opposite migration occurences towards \textit{TestNG}, all the efforts have been provided within one \textit{commit} day : one commit for 8 projects, and 2, 3 and 8 commits for the 3 remaining. 
%
%Similar trends were identified on the 11 projects that migrated to \textit{Mockito}. One needed one person, and 5 commits on 3 days to achieve the migration from \textit{JMock}. An other one required 2 persons, 3 days covering 7 commits to fully withdraw \textit{JMock} from the project. One project needed 9 commits, 2 persons and 5 \textit{commit} days to make \textit{EasyMock} disappear. The 8 remaining projects all completed their respective migration within one commit. 
%
%For the JSON facilities, the 15 migrations studied have been completed in one commit, except for one that was made within 2 commits. In all the scenarios where more than 1 commit was necessary, investigation on commit logs did not unfortunately reveal any details on efforts or obstacles encountered by developers.
%
%To answer to \textsc{RQ6}, our sample analysis showed that the most common development pratice is to migrate the source code within one commit. In our case study, 63 out of 76 migrations (i.e., 83\%) were in this situation. However, in some cases a coexistence happen but it rarely goes beyond 10 commits. Reasons for this time are not clear yet, and we cannot conclude that developers face issues and challenges during their migrations. While source code transformations seem less tedious with loggers framework, other type of libraries such as testing or mocking may require more time, seem their API design differ and require more structural code modifications (i.e., annotations).
%
%We also learn that migrations cannot be detected if our sampling methodology sets a too low interval, e.g. 1 commit, as discussed in Section \ref{sec:study}. Indeed, periods of library cohabition are not detected using such interval.


